Well begun is half done: the computation of Eulerian paths

We characterize the uniform computational strength of finding (one-way or two-way, directed or undirected) Eulerian paths in countable graphs. In the one-way case, for both directed and undirected graphs, this problem is Weihrauch-equivalent to $\mathsf{lim}\times\mathsf{C}_{\mathbb{N}}'$, where $\mathsf{C}_{\mathbb{N}}'$ is the jump of closed choice on the natural numbers. This refines the proof-theoretic strength of the existence of a one-way Eulerian path given by the reverse mathematics framework. The $\mathsf{C}_{\mathbb{N}}'$ component comes entirely from the difficulty of choosing a starting vertex: with a valid start prescribed, the problem is equivalent to $\mathsf{lim}$, which also characterizes the degree of the two-way directed/undirected Eulerian path problem. We also study the complexity of orienting the edges of a graph while preserving the existence of a one-way/two-way Eulerian path. In the one-way case, this problem is not computable, and we prove that $\mathsf{lim}_2<_{\mathrm{W}}\mathsf{OrientEP}<_{\mathrm{W}}\mathsf{C}_{2}'\sqcap\mathsf{Sort}_2$ and $\mathsf{OrientEP}\not\le_{\mathrm{W}}\mathsf{C}_{\mathbb{N}}$. On the other hand, valid orientations are uniformly computable for two-way paths and for one-way paths with a prescribed valid starting vertex.

==> symbols.tex <==
\usepackage{ifthen}
\usepackage{xargs}

\usepackage{xcolor}

\makeatletter


\newcommand{\textdef}[1]{{\normalfont\textit{#1}}}

\newcommand{\st}{{}\,:\,{}}
\newcommand{\set}[2]{\{ #1 \st #2\} }


\def\function{\@ifstar\@function\@@function}
\newcommand{\@function}[2]{#1 \to #2}
\newcommand{\@@function}[2]{\colon #1 \to #2}

\def\mfunction{\@ifstar\@mfunction\@@mfunction}
\newcommand{\@mfunction}[2]{#1 \rightrightarrows #2}
\newcommand{\@@mfunction}[2]{\colon #1 \rightrightarrows #2}

\newcommand{\restrict}[1]{\ensuremath{\left. \hspace{-1mm} \right|_{#1}}}


\newcommand{\pfunction}[2]{:\subseteq #1 \to #2}
\newcommand{\pmfunction}[2]{:\subseteq #1 \rightrightarrows #2}

\newcommand{\id}{\operatorname{id}}

\newcommand{\length}[1]{|{#1}|}
\newcommand{\prefix}{\sqsubseteq}
\newcommand{\pprefix}{\sqsubset}
\newcommand{\extend}{\sqsupseteq}
\newcommand{\pextend}{\sqsupset}


\newcommand{\Baire}{\mathbb{N}^\mathbb{N}}
\newcommand{\baire}{\mathbb{N}^{<\mathbb{N}}}
\newcommand{\Cantor}{2^\mathbb{N}}
\newcommand{\cantor}{2^{<\mathbb{N}}}
% \newcommand{\Graphs}{\mathrm{Gr}}
% \newcommand{\BGraphs}{\mathrm{Gr}}

\newcommand{\turingreducible}{\le_\mathrm{T}}
\newcommand{\turingequiv}{\equiv_\mathrm{T}}
\newcommand{\strictlyturingreducible}{<_\mathrm{T}}
\newcommand{\turingincomparable}{\,|_\mathrm{T}\,}


\newcommand{\weireducible}{\le_{\mathrm{W}}}
\newcommand{\weige}{\ge_{\mathrm{W}}}
\newcommand{\strictlyweireducible}{<_\mathrm{W}}
\newcommand{\strictlyweiabove}{>_\mathrm{W}}
\newcommand{\weiequiv}{\equiv_{\mathrm{W}}}
\newcommand{\weiincomparable}{~|_{\mathrm{W}~}}

\newcommand{\sequence}[2]{(#1)_{#2}}
\newcommand{\family}[2]{\{#1\}_{#2}}

\newcommand{\str}[1]{({#1})}

\newcommand{\coding}[1]{\langle #1 \rangle}
\newcommand{\pairing}[1]{\coding{#1}}
\newcommand{\concat}{\smash{\raisebox{.9ex}{\ensuremath\smallfrown} }}

\newcommand{\dom}{\operatorname{dom}}
\newcommand{\ran}{\operatorname{ran}}

\newcommand{\parallelization}[1]{\widehat{#1}}

\newcommand{\Deg}{\mathsf{Deg}}
\newcommand{\DegLF}{\mathsf{Deg}_{\mathrm{LF}}}

\newcommand{\outdeg}{\mathrm{out}}
\newcommand{\indeg}{\mathrm{in}}

\newcommand{\mflim}{\mathsf{lim}}
\newcommand{\boldfacePi}{\boldsymbol{\Pi}}
\newcommand{\boldfaceSigma}{\boldsymbol{\Sigma}}
\newcommand{\CNatural}{\mathsf{C}_{\mathbb{N}}}
\newcommand{\UCNatural}{\mathsf{UC}_{\mathbb{N}}}
\newcommand{\sTCN}{\mathsf{sTC}_{\mathbb{N}}}
\newcommand{\LPO}{\mathsf{LPO}}

\newcommand{\EP}{\mathsf{EP}}
\newcommand{\EPstart}{\EP_{\mathrm{start}}}
\newcommand{\DEP}{\mathsf{DEP}}
\newcommand{\DEPstart}{\DEP_{\mathrm{start}}}

\newcommand{\TEP}{\mathsf{EP}_2}
\newcommand{\TDEP}{\mathsf{DEP}_2}

\newcommand{\OrientOW}{\mathsf{OrientEP}}
\newcommand{\OrientTW}{\mathsf{OrientEP}_2}
\newcommand{\Choice}[1]{\mathsf{C}_{#1}}
\newcommand{\Sort}{\mathsf{Sort}}

\newcommand{\AoUC}{\mathsf{AoUC}_{\mathbb{N}}}
\newcommand{\mfliminf}{\mathsf{liminf}}
\newcommand{\strongT}[1]{\mathsf{sT}(#1)}
\newcommand{\totalization}[1]{\mathsf{T}(#1)}
\makeatother

